Translation between Molecules and Natural Language

We present $\textbf{MolT5}$ $-$ a self-supervised learning framework for pretraining models on a vast amount of unlabeled natural language text and molecule strings. $\textbf{MolT5}$ allows for new, useful, and challenging analogs of traditional vision-language tasks, such as molecule captioning and text-based de novo molecule generation (altogether: translation between molecules and language), which we explore for the first time. Since $\textbf{MolT5}$ pretrains models on single-modal data, it helps overcome the chemistry domain shortcoming of data scarcity. Furthermore, we consider several metrics, including a new cross-modal embedding-based metric, to evaluate the tasks of molecule captioning and text-based molecule generation. Our results show that $\textbf{MolT5}$-based models are able to generate outputs, both molecules and captions, which in many cases are high quality.

==> 3data.tex <==

\section{Data}

A primary difficulty of training joint molecule-text representations is the scarcity of training data pairs. Thus, to train MolT5 requires different sources of data, some of which are large quantities of single-modal data, in addition to the gold standard molecule-description pairs for finetuning. 

For large-scale natural language data, we use the ``Colossal Clean Crawled Corpus'' (C4) \cite{raffel2019exploring}. For the molecule data, we use 100 million SMILES strings from the ZINC-15 dataset \cite{sterling2015zinc} which were used in Chemformer \cite{irwindimitriadishebjerrum2021}.

For our gold standard data, we use ChEBI-20, which was first presented in \cite{edwards2021text2mol}. It consists of 33,010 molecule-description pairs, which are separated into 80/10/10\% train/validation/test splits. In this paper, we work with SMILES strings, so we remove 2 molecules represented by the wildcard SMILES string: ``*''. This dataset is also used to train the baseline models. Further, many of the captions contain a name for the molecule at the start of the string. To force the molecule to focus on the semantics of the description, we replace the molecule's name with "The molecule is [...]". 











